Hindsight Planner: A Closed-Loop Few-Shot Planner for Embodied Instruction Following

This work focuses on building a task planner for Embodied Instruction Following (EIF) using Large Language Models (LLMs). Previous works typically train a planner to imitate expert trajectories, treating this as a supervised task. While these methods achieve competitive performance, they often lack sufficient robustness. When a suboptimal action is taken, the planner may encounter an out-of-distribution state, which can lead to task failure. In contrast, we frame the task as a Partially Observable Markov Decision Process (POMDP) and aim to develop a robust planner under a few-shot assumption. Thus, we propose a closed-loop planner with an adaptation module and a novel hindsight method, aiming to use as much information as possible to assist the planner. Our experiments on the ALFRED dataset indicate that our planner achieves competitive performance under a few-shot assumption. For the first time, our few-shot agent's performance approaches and even surpasses that of the full-shot supervised agent.

==> previous_version/intro_old.tex <==
\section{Introduction}
With the development of AI and robotics, many previous works have combined them together to handle Embodied Instruction Following(EIF) tasks \citep{ALFRED}. In such task, agent will be given a human instruction(eg.``Put a heated mug down on a table'') and egocentric visual observation at each step. Agent are required to output low-level actions(eg. MoveAhead, RotateRight, etc.) based on the observation to finish the task. These task are usually challenge due to the sparse reward. For such reason, many works have adopted hierarchical structure to deal with it\citep{LLMplanner,FILM,HLSM,CAPEAN}. The high-level module decompose the whole task into several sub-tasks, the low-level module outputs actions to finish each sub-task. Previously, subgoal planner are trained on human-annotated dataset through supervised learning.However, they require large amounts of data and usually have weak robust ability \citep{FILM,HLSM,CAPEAN}.

Recently with the advancements in Large language models(LLMs), many research has explored utilizing LLM as subgoal planner with respect to the In-Context Learning ability of LLM \citep{LLMplanner,Socraticplanner,ahn2022icanisay}. Though these methods achieved competitive performance in few-shot assumption, a crucial drawback is that the In-Context-Examples could not provide enough information for the agent.From an RL perspective, these examples usually focus on exploitation and neglect exploration, which is a crucial part of Reinforcement Learning. This imbalance can prevent the agent from developing robust abilities. For instance, once the agent execute a sub-optimal action, the agent will face a out-of-distributed state, and the agent fail to know how to correct it, lead to the failure of the task.

previous work, such as  \cite{min2022rethinkingroledemonstrationsmakes}, shows that the choice of demonstration has little impact on the performance of large language models (LLMs). However, these works are valid for one-step tasks, such as classification or multiple-choice tasks. In long-horizon reinforcement learning (RL) tasks, the situation is quite different, as the gap grows exponentially. Assume that after In-Context Learning, the distribution of the agent's actions gets closer to that of the Oracle's, with an accuracy of 0.9. In a one-step task, the performance difference between the suboptimal agent and the Oracle is  10\%. However, in a 10-step RL task, the gap become $1-0.9^{10}=65.1\%$
 


Inspired by RAFA \citep{RAFA}--the first time framework achieve provable sample efficiency guarantees in autonomous LLM agents by constructing mapping between RL and LLM--we proposed a novel agent that further apply Hindsight into LLM.

The Hindsight planner contains three components: Adaptation Model, Hindsight Prompts Constructor and Task Planner. The Adaptation model \citep{kumar2021rmarapidmotoradaptation} utilizing LLM to predict the PDDL parameters that are invisible for the agent in validation and test phase. The Task planner is a hierarchical framework where the high-level controller is instanced by RAFA \citep{RAFA} . The low-level controller following previous research for fair comparison,is instanced by the Hierarchical Language-conditioned Spatial Model \citep{HLSM}.  The Hindsight Prompts Constructor first instance  the agents with ground truth samples retrieved from training dataset and run the agent on those trajectory ,collecting the real, sub-optimal rollouts from environment. After that, we relabel those rollouts to make them could not only provide guidance of how to finish the task but also include how to handle with incorrect actions, we append the relabeled rollouts with the origin ground truth rollouts and instanced the hindsight planner with new samples pool.
% Try to intergrate adapt model, hindsight together?
 In summary, our contributions are three-fold:
 
 1.We first designed a closed-loop high-level planner, the hindsight planner, which incorporates hindsight prompting and an adaptation module using LLMs in ALFRED \citep{ALFRED}.
 % \zsa{Is it better to describe the first contribution as proposing the xxx agent that contains xx and yy? The second contribution is how the xx and/or yy works (add more details to the current point 2). The third contribution is we applied the agent to Alfred and experiments show the results are SOTA (including the numbers of SR etc).}
 % Need to change
 
 2.Our novel framework provides robust performance in Embodied Instruction Following (EIF) tasks. The adaptation module enables the agent to adjust its predictions as it explores the environment, and hindsight prompts allow the agent to revise suboptimal actions.
 
 3.We applied our agent to ALFRED, and experiments show that our results achieve state-of-the-art (SOTA) under few-shot assumptions, with success rates of 25.51 and 18.77 in the ``Test Seen'' and ``Test Unseen'' splits, respectively.
 \begin{figure}[H]
\centering

\includegraphics[width=\textwidth]{figs/demo2.png}  
\caption{\small 
\textbf{Left}: the illustration of hindsight planner.At each time step $t$, the Actor is prompted with both the ground truth (GT) samples and the hindsight samples, and the Actor makes decisions separately based on these samples. The Critic is utilized to evaluate the actions. The best rollout $(s_t,a_t^*,s_{t+1}^*,a_{t+1}^*\ldots)$ will be selected and return $a_t^*$ \textbf{Right}: an example of the relabeling process of Actor: after collecting suboptimal rollouts, the LLM is prompted to generate a reflection on the suboptimal actions taken. Following this reflection, the LLM is then asked to complete the suboptimal rollout.
\vspace{-0.1cm}}
\label{fig:demo2}

% \zsa{Left: Explain why this is not what we what (add 10-step 0.9 example). Middle: The blue arrow should be something that indicates 'motivates'. Right: Not very clear what 'relabel samples' means, should add more details.}

\end{figure}


==> previous_version/method_old.tex <==
\section{Hindsight Planner}
\begin{algorithm}[h]\small
	\caption {Hindsight Planner}
	\begin{algorithmic}[1]	\label{alg:llm}
 
 
    \STATE \textbf{Input:} An LLM-planner $\texttt{LLM-PL}$, an adaptation module $Adapter$, task instruction  $I$, observed Objects $O= \emptyset$, sub-goal History $G=\emptyset$,current Sub-goal  $S=\emptyset$,time step $t\leftarrow 0$,sub-goal index $k\leftarrow 0$
    \STATE Get samples pool $D$ and initialize  ${Actor}_{\theta}$,  ${Critic}$,$ {Adapter}$ from $D$.  $~\theta\in \{gt,hind\}$ \hfill \cref{alg:collection}
 
    \WHILE{Not \textit{Finished}}
        \STATE Get PDDL arguments $P$ $\leftarrow$ ${Adapter}(I,O)$
        \STATE Plan and get sub-goal $S_k\leftarrow$  \texttt{LLM-PL}(${Actor}_{gt}, {Actor}_{hind},{Critic},P,I,O,G$) \hfill\cref{alg: example}
          \STATE Set $S_k$ as sub-goal for \texttt{Low-PL} 
        \WHILE{ $S_k$ not \textit{Finished} and not \textit{Failed} }
            \STATE Invoke \texttt{Low-PL} to plan and execute $a_t$ and update $O$
            \STATE $t\leftarrow t+1$
            
            \IF{$S_k$ \textit{Finished}}
                \STATE  $G$.insert($S_k$)
                \STATE $k\leftarrow k+1$ 
              
            \ENDIF
        \ENDWHILE
 
        
    \ENDWHILE
	\end{algorithmic}
\end{algorithm}
\subsection{Overview}


 
The hindsight planner is instantiated with LLMs, in \cref{prompt_design}, We then further discuss the components of the planner. The hindsight planner consists of several components: a samples pool, an adaptation module, and a task planner. At each time step $t$, hindsight planner receives object lists $O_t$ from observation functions \citep{HLSM}. The adaptation module, as described in \cref{adapt_model}, predicts the latent PDDL arguments $P$ for the task. The whole state $s_t$  constructed by the observed object lists and predicted PDDL arguments. The actor-critic task planner $\texttt{LLM-PL}$ generates a future trajectory over a long horizon and returns sub-goal $S_k$ based on $x_t$. In \cref{hindsight} we discuss the initialization process of $\mathit{Actors}$ and $Critic$ and the details of the reasoning process of $\texttt{LLM-PL}$  is shown in \cref{task_planner}.To ensure that the output from LLMs meets the requirements, a frozen BERT \citep{BERT} model is used to map the output to the nearest action-object pairs. The proposed sub-goal will be executed by a low-level controller \texttt{Low-PL}  \citep{HLSM}. When a sub-goal is completed or fails, the LLM planner reinvokes the reasoning process to replan another future trajectory from the new state. The whole algorithm is shown in \cref{alg:llm}.




 
\subsection{Prompt Design}
\label{prompt_design}
All components follow a similar design. The prompt begins with an intuitive explanation of the task and a role description of the LLMs. A frozen BERT is then used as a kNN retriever, encoding the task description and selecting the $K$ examples with the closest Euclidean distance from the samples pool as in-context samples. \citep{LLMplanner} Intuitively, the planner would make similar suboptimal actions in similar tasks. For instance, if in an in-context sample ``Place two spray bottles into the cabinet,'' the planner fails to open the cabinet when putting the second spray bottle into it, in the current task ``Putting two candles in a cabinet'', the planner would know to avoid a similar mistake.
\subsection{Adaptation Module}
\label{adapt_model}

Adaptation module aims to predict the latent variable from observed objects. The input prompts for the adaptation module begin with an intuitive explanation of ALFRED. This is followed by several in-context examples. At the end of the prompt is the current task and object list. At each step, the object list is updated as the planner explores the environment. 

% We do not include past actions in the prompts like \cite{kumar2021rmarapidmotoradaptation}, so that the adapt model can be separated from the task planner, making the entire framework more robust.

The output content from the adaptation module varies depending on the task description. Inspired by PDDL \citep{PDDL,PDDL_in_LLM} in the trajectory of ALFRED, in practice, the adaptation module needs to predict the following arguments at each step: (1) \textit{object\_target}: The specific object that will be interacted with in the task. (2) \textit{parent\_target}: The final place for the object in the task. (3) \textit{mrecep\_target}: The container or vessel required for the task. (4) \textit{toggle\_target}: The device that needs to be toggled in the task. (5) \textit{object\_state}: Indicates whether the target object needs to be cleaned, heated, or cooled. (6) \textit{object\_sliced}: Determines if the object needs to be sliced. (7) \textit{two\_object}: Specifies whether the task requires the planner to handle and place two objects. The adaptation module predicts these arguments at each step before reasoning, and then the arguments are processed into a certain format so they can be better understood by the task planner.
\subsection{Hindsight Prompt}
\label{hindsight}
\begin{figure}[H]
\centering
\includegraphics[width=\textwidth]{figs/demo1.png}  
\caption{\small comparison of Hindsight planner and previous supervised method when taking suboptimal actions. Agent pick up the incorrect object(``Basketball'') at the first time. In supervised method, planner fail to handle  this situation, leading to the failure of the task. In contrast, the hindsight planner can adjust from the incorrect action and successfully complete the task.\vspace{-0.1cm}}
\label{fig:demo1}
\end{figure}


The Hindsight prompt consists of two main parts: the collection phase and the deployment phase. During the collection phase, the planner executes tasks and retrieves $K $ examples from a small set of ground truth training examples. At each task, the planner generates a probable suboptimal trajectory and relabels them. The algorithm can be viewed in \cref{alg:collection}. During the deployment phase, both ground truth samples and hindsight samples are used to prompt the planner. 

 

We give a further discussion on the relabeling process. The relabeling process utilizes the reasoning ability of LLMs to fit suboptimal trajectories into correct rollouts. The input content includes the ground truth trajectory from training data, the task description, and the suboptimal trajectory. For the prompt of the Critic model, LLMs are required to generate the critique based on the ground truth trajectory. For the prompt of the Actor model, LLMs are required to generate a reflection on the mistakes in the suboptimal trajectory and then generate actions based on this reflection. A example can be viewed in \cref{fig:demo2}. However, directly applying the task description from ALFRED can lead to unsatisfactory results, as the task description is often vague. For example, the task ``Put a chilled potato on the small black table'' requires the planner to put the \textit{potato} on a \textit{SideTable}. If the task description is applied directly, LLMs might focus on the \textit{black table} and return the incorrect action ``PutObject BlackTable''. If the task description is not included in the prompt, it could lead LLMs to simply imitate the ground truth trajectory. However, planner usually have multiple choices to complete a task. For instance, in a task requiring the planner to slice an apple, after slicing the apple, the planner could put the \textit{Knife} on the \textit{DiningTable} or \textit{CounterTop}. To address this issue, we relabel the task based on the latent PDDL arguments. Thus, the task description "Put a chilled potato on the small black table" would become "Pick up one cooled potato and put it on the SideTable". This approach helps to clarify the task for the planner and reduces the ambiguity in the instructions.

\subsection{Task Planner}
\label{task_planner}
We adopt an Actor-Critic planner \citep{RAFA}. At each time step $ t $, the planner receives $ s_t $ from the environment and the adaptation module. We initiate two Actors: $ Actor_{gt} $ and $ Actor_{hind} $, with different samples from the samples pool $ D $. For each state, we require each Actor to generate $ \frac{W}{2} $ actions. The Critic then selects the best $ B $ actions. A generator $ \psi $ generates the next state based on each action. In this way, we map the $\mathit{Actors}$ and $Critic$ into $ B $ future trajectories and select the best future trajectory $ (s_t, a_t^*, \ldots) $ through the Critic. $ a_t^* $ is then returned as the sub-goal for \texttt{Low-PL}. The intuition behind having two Actors is that we hope the planner learns from the ground truth trajectories to make correct decisions each time, and when a suboptimal action is taken, we also hope the planner learns how to correct it. \cref{fig:demo2} shows the reasoning process of the planner,  \cref{alg: example} provides a detailed algorithm.



% we require the Actor to output $W$ actions each time, with half of the $W$ actions using ground truth samples as in-context samples, while the other half use relabeled suboptimal samples as in-context samples. The Critic is prompted with relabeled suboptimal samples and evaluates each action. Intuitively, this approach aims to balance path length and robustness: 
 




% An Actor model instanced by LLM \texttt{Actor}, a Critic model instanced by LLM \texttt{Critic},

==> previous_version/relatework_old.tex <==
\section{Related Work}
% turn into related work
\subsection{Large Language Model (LLM) and In-Context Learning (ICL)}
Large language models (LLMs) have shown incredible reasoning ability \citep{attention,Emergent_Abilities,Llama,gpt4} across a wide range of tasks. A crucial way to activate this reasoning ability is through In-Context Learning (ICL) \citep{llm_few_shot_learner,ICL_servey}, which allows LLMs to solve complex tasks with only a few samples, without the need for fine-tuning, which can be time-consuming and computationally expensive. To better utilize the ICL ability, many works have proposed certain frameworks to improve reasoning ability \citep{TOT,COT,GOT}. Among them, \cite{RAFA} proposed a novel perspective by bridging RL and LLM, which inspired us to view ICL from an RL aspect. \cite{ICL_explanation} interprets ICL as Implicit Bayesian Inference, while \cite{dai2023gptlearnincontextlanguage} believes that ICL is performing implicit Gradient Descent. All of these imply the importance of content in ICL, an area that has been the focus of several works. To address this, we propose the use of hindsight prompts method to fill in the gap.
\subsection{adaptation module}
Adaptation modules have been proven to work effectively in legged robots \citep{kumar2021rmarapidmotoradaptation,5655cf7f69e149148a2ea1c5a664b4ba,peng2020learningagileroboticlocomotion}. These modules aim to bridge the gap between simulation and the real world, often trained through supervised learning to predict crucial information that robots can sense in simulators but not in the actual world, such as surface friction or the payload of the robot. The base policy then makes decisions based on sensor information and the invisible information predicted by the adaptation module. Inspired by this, we hope our adaptation models can bridge the gap between vague language instructions and clear subgoals of the task. For instance, the task ``Put a soap bottle on the small black table'' requires the agent  to put the \textit{SoapBottle} on the \textit{SideTable}. The adaptation model aims to link the concept of ``SideTable'' with ``small black table'' for the agent. To achieve this, the LLMs are prompted to predict the invisible PDDL arguments in each task.

% Previous work\cite{kumar2021rmarapidmotoradaptation},\cite{5655cf7f69e149148a2ea1c5a664b4ba},\cite{peng2020learningagileroboticlocomotion}  usually aims to predict a low-dimensional latent embedding because predicting the exact privileged information is typically challenging. However, with the reasoning capabilities of Large Language Models (LLMs),we directly predict the PDDL\cite{PDDL} arguments, as it could achieve satisfactory performance while ensuring that the predictions are also understandable to humans. 

Previous works, such as \cite{FILM}, train a BERT \citep{BERT} to predict the PDDL arguments and decompose high-level instructions into template subgoals. However, our approach differs from theirs in two aspects. (1) Previous work simply decomposes the instruction at the beginning of the task, whereas our adapt model predicts the key arguments at each time before reasoning, allowing the prediction to change as the agent explores the environment, which make our agent more robust. For example, in the task \textit{``Move a coffee cup from the round table to the small table''}, the adapt model might initially predict \textbf{Cup} as the target object. With more exploration of the environment, the agent does not find a \textbf{Cup} but finds a \textbf{Mug} instead, then the adapt model would adjust its prediction to \textbf{Mug}. While both object are legal in the task. 
(2) We do not apply type templates directly. While the adapt model predicts PDDL arguments, it only assists the task planner in making decisions, which makes our method more general. Results show that our method can achieve competitive performance even without the assistance of the adapt model \cref{tab:3}.
\subsection{Hindsight in LLM}
Hindsight algorithms \citep{andrychowicz2018hindsightexperiencereplay,li2020generalizedhindsightreinforcementlearning,pong2020temporaldifferencemodelsmodelfree}, are widely adopted in the reinforcement learning (RL) area. In general, the hindsight method 'uses future state information to automatically mine for positive, or ``optimal'', examples with respect to certain contextual parameter values, where these examples can accelerate RL or be used for behavior cloning (BC)' \citep{furuta2022generalizeddecisiontransformeroffline}. Typically, hindsight is used to help improve the performance of trained RL algorithms. \cite{furuta2022generalizeddecisiontransformeroffline} applied the hindsight method in training a Transformer model and achieved competitive performance on several Baselines. However, training a model from scratch usually requires a large amount of data. In contrast, In-Context Learning (ICL), utilizing the reasoning ability of Large Language Models (LLMs), allows an agent to complete a complex task with only a few samples. \cite{dai2023gptlearnincontextlanguage} has shown that ICL executes an implicit parameter update; therefore, we decide to apply the hindsight method through ICL.

The Hindsight  prompt in our method  consists of two main parts: the collection phase and the relabeling phase. During the collection phase, the agent executes tasks and retrieves\textbf{ K} examples from a small set of ground truth training examples. The agent makes decisions based on the In Context Learning (ICL) examples and the current environmental information.  At each task, the agent generates a probable sub-optimal trajectory. After collecting the trajectories, we use Large Language Models (LLMs) to relabel the sub-optimal trajectories for both the actor and the critic. The relabeling process corrects the trajectory to achieve the desired outcome. For example: ``Wash a pan and put it away'' requires agent to wash a \textit{Pan} and put it on the \textit{DiningTable}. The sub-optimal trajectory from agent is:
\{(PickupObject , Pan), (PutObject , Sink),  (ToggleObjectOn , Faucet), (PickupObject , Pan), (PutObject , CoffeeMachine)\}.
Note that in this example, the agent fails to put the Pan in the correct location and does not turn off the faucet. The corrected trajectory for the task should be: \{(PickupObject , Pan), (PutObject , Sink),  (ToggleObjectOn , Faucet), (PickupObject , Pan), (PutObject , CoffeeMachine), (ToggleObjectOff , Faucet), (PickupObject ,Pan), (PutObject, DiningTable)\}
This relabeling process helps to guide the agent towards optimal behavior by providing a corrected sequence of actions that align with the task's goal. The agent can then learn from these corrected trajectories to improve its performance on similar tasks in ``valid/test'' splits.

%reflection etc.

==> prompt/criticsamples.tex <==
Task:Place a cup in the coffee maker.
**Your knowledge about this task** is: I need to pick up one Mug first. Then I should put the Mug in fridge to cool it. *Important:Note that I don't need to turn on the fridge and the fridge is initially closed. After thatm I should pick up Mug from fridge . Then I should put Mug in/on the CoffeeMachine. 
**actions**:
The objects you have seen are: Bowl, Bread, ButterKnife, Cabinet, Chair, CoffeeMachine, CounterTop, Cup, DishSponge, Drawer, Fridge, GarbageCan, Lettuce, LightSwitch, Microwave, Mirror, Mug, Pan, PepperShaker, Plate, SaltShaker, Sink, SoapBottle, Spatula, Spoon, StoveBurner, StoveKnob, DiningTable, SideTable, Toaster, Window
 OpenObject : Cabinet
>OK
 PickupObject : Cup
>OK
 CloseObject : Cabinet
>OK
 PutObject : DiningTable
>OK
 PutObject : CoffeeMachine
>OK
Based on the **actions** and **Your knowledge about this task** , write a Critic.
Critic:In this task, I need to do the following things in order: open the cabinet, pick up a mug, close the cabinet, place the mug in the fridge to cool it, open the fridge, pick up the cooled mug, close the fridge, and put the mug on the coffee machine. There are 7 subgoals in all, I achieved 1 of them, this is because I picked up a cup instead of a mug, I did not put the mug into the fridge to cool it down, and I did not place the cooled mug on the coffee machine. Additionally, I put the object on the dining table which was not required in the task. Therefore, most of my actions were incorrect. The value is 1/7=0.14.

Task:Warm a cup to make coffee
**Your knowledge about this task** is: I need to pick up one Mug first. Then I should use microwave to heat the Mug.*Important:Note that I need to turn on and turn off the microwave and the microwave is initially closed. After that I should pick up Mug from microwave .Then I should put Mug in/on the CoffeeMachine. 
**actions**:
 PickupObject : Cup
>OK
 OpenObject : Microwave
>OK
 PutObject : Microwave
>OK
 CloseObject : Microwave
>OK
Based on the **actions** and **Your knowledge about this task** , write a Critic.
Critic:In this task, I need to do the following things in order: Open the fridge, pick up the mug, close the fridge, open the microwave, put the mug into the microwave, close the microwave, turn on the microwave, turn off the microwave, open the microwave, pick up the heated mug, close the microwave, and put the heated mug on the coffee machine. There are 11 subgoals in order, my current state achieved 0 of them, because the agent did not follow the correct sequence of actions, missing the initial step of opening the fridge and instead picking up a different cup not specified in the subgoals. The value is 0/11=0.00.

